ESBMC-Jimple: Verifying Kotlin Programs via Jimple Intermediate Representation

In this work, we describe and evaluate the first model checker for verifying Kotlin programs through the Jimple intermediate representation. The verifier, named ESBMC-Jimple, is built on top of the Efficient SMT-based Context-Bounded Model Checker (ESBMC). It uses the Soot framework to obtain the Jimple IR, representing a simplified version of the Kotlin source code, containing a maximum of three operands per instruction. ESBMC-Jimple processes Kotlin source code together with a model of the standard Kotlin libraries and checks a set of safety properties. Experimental results show that ESBMC-Jimple can correctly verify a set of Kotlin benchmarks from the literature and that it is competitive with state-of-the-art Java bytecode verifiers. A demonstration is available at https://youtu.be/J6WhNfXvJNc.

==> BMC of Kotlin Programs Using Jimple (Copy)/authors.tex <==
\author{Rafael Sá Menezes}
\orcid{0000-0002-6102-4343}
\affiliation{
  \institution{University of Manchester}
  \country{United Kingdom}
}
\additionalaffiliation{
  \institution{Federal University of Amazonas}
  \country{Brazil}
}

\author{Daniel Yuri da Rocha Moura}
\affiliation{%
  \institution{Federal University of Amazonas}
  \country{Brazil}
}

\author{Helena F. Cavalcante}
\affiliation{%
 \institution{Federal University of Amazonas}
 \country{Brazil}
 }

\author{Rosiane de Freitas Rodrigues}
\affiliation{%
  \institution{Federal University of Amazonas}
  \country{Brazil}}

\author{Lucas C. Cordeiro}
\orcid{0000-0002-6235-4272}
\affiliation{%
  \institution{University of Manchester}
  \country{United Kingdom}
}
\additionalaffiliation{
  \institution{Federal University of Amazonas}
  \country{Brazil}
}


\author{Rafael Sá Menezes}
\orcid{0000-0002-6102-4343}
\additionalaffiliation{
  \institution{Federal University of Amazonas}
  \country{Brazil}
}
\author{Lucas C. Cordeiro}
\orcid{0000-0002-6235-4272}
\additionalaffiliation{
  \institution{Federal University of Amazonas}
  \country{Brazil}
}
\affiliation{%
  \institution{University of Manchester}
  \country{United Kingdom}
}


\author{Daniel Yuri da Rocha Moura}
\author{Helena F. Cavalcante}
\author{Rosiane de Freitas Rodrigues}
\affiliation{
  \institution{Federal University of Amazonas}
  \country{Brazil}
}


==> BMC of Kotlin Programs Using Jimple (Copy)/bck.tex <==

Figure~\ref{lst:example} contains an example of the full convertion
process. At the left, the Listing~\ref{lst:kotlin} contains the
source code of a Kotlin class, the \texttt{Foo} class contains a 
private member \texttt{member} containing getters and setters. The class also contains a function \texttt{increment} which adds \texttt{member} by a given number and return its value. After its
convertion into Jimple in Listing~\ref{lst:jimple} we can see the 
generated code, containing intermediate variables and member calls.
The Jimple example was simplified for better readability (removed getter/setters and final modifiers).
Finally, at Listing~\ref{lst:goto} we see the program in GOTO.

\begin{figure*} % [htp]
% Let's make this an lstlisting, not a figure...
\begin{lrbox}{}
\begin{lstlisting}[language=kotlin, style=nasm, xrightmargin=.6667\linewidth]
class Foo(var member: Int) 
{
  fun increment(N: Int): Int
  {
    member = member + N
    return member
  }
}

\end{lstlisting}
\end{lrbox}
\subcaptionbox{Kotlin Code\label{lst:kotlin}}{\usebox{\verbsavebox}}\hfill%
\begin{lrbox}{\verbsavebox}
\begin{lstlisting}[language=jimple, style=nasm, xrightmargin=.6667\linewidth]
public class Foo
{
  private int member;
  ...
  public int increment(int)
  {
    Foo r0;
    int i0, $i1, $i2, $i3;
    r0 := @this: Foo;
    i0 := @parameter0: int;
    $i1 = r0
      .<Foo: int member>;
    $i2 = $i1 + i0;
    r0.<Foo: int member>
      = $i2;
    $i3 = r0
      .<Foo: int member>;
    return $i3;
  }
}
\end{lstlisting}
\end{lrbox}
\subcaptionbox{Jimple Code (simplified)\label{lst:jimple}}{\usebox{\verbsavebox}}\hfill%
\begin{lrbox}{\verbsavebox}
\begin{lstlisting}[xrightmargin=.6667\linewidth]
trait Sys {
  type ID <: Ident[Tx]
  type Tx
}

trait Muta[S <: Sys] {
  // evidence required:
  val s: S
  def id: s.ID
  // well defined:
  def dispose(tx: s.Tx) =
    id.dispose(tx)
}
\end{lstlisting}
\end{lrbox}
\subcaptionbox{GOTO Code\label{lst:goto}}{\usebox{\verbsavebox}}
\caption{Kotlin into GOTO convertion\label{lst:example}}
\end{figure*}

==> authors.tex <==
\author{Rafael Sá Menezes}
\orcid{0000-0002-6102-4343}
\affiliation{
  \institution{University of Manchester}
  \country{United Kingdom}
}
\additionalaffiliation{
  \institution{Federal University of Amazonas}
  \country{Brazil}
}

\author{Daniel Yuri da Rocha Moura}
\affiliation{%
  \institution{Federal University of Amazonas}
  \country{Brazil}
}

\author{Helena F. Cavalcante}
\affiliation{%
 \institution{Federal University of Amazonas}
 \country{Brazil}
 }

\author{Rosiane de Freitas Rodrigues}
\affiliation{%
  \institution{Federal University of Amazonas}
  \country{Brazil}}

\author{Lucas C. Cordeiro}
\orcid{0000-0002-6235-4272}
\affiliation{%
  \institution{University of Manchester}
  \country{United Kingdom}
}
\additionalaffiliation{
  \institution{Federal University of Amazonas}
  \country{Brazil}
}


\author{Rafael Sá Menezes}
\orcid{0000-0002-6102-4343}
\additionalaffiliation{
  \institution{Federal University of Amazonas}
  \country{Brazil}
}
\author{Lucas C. Cordeiro}
\orcid{0000-0002-6235-4272}
\additionalaffiliation{
  \institution{Federal University of Amazonas}
  \country{Brazil}
}
\affiliation{%
  \institution{University of Manchester}
  \country{United Kingdom}
}


\author{Daniel Yuri da Rocha Moura}
\author{Helena F. Cavalcante}
\author{Rosiane de Freitas Rodrigues}
\affiliation{
  \institution{Federal University of Amazonas}
  \country{Brazil}
}


==> bck.tex <==

Figure~\ref{lst:example} contains an example of the full convertion
process. At the left, the Listing~\ref{lst:kotlin} contains the
source code of a Kotlin class, the \texttt{Foo} class contains a 
private member \texttt{member} containing getters and setters. The class also contains a function \texttt{increment} which adds \texttt{member} by a given number and return its value. After its
convertion into Jimple in Listing~\ref{lst:jimple} we can see the 
generated code, containing intermediate variables and member calls.
The Jimple example was simplified for better readability (removed getter/setters and final modifiers).
Finally, at Listing~\ref{lst:goto} we see the program in GOTO.

\begin{figure*} % [htp]
% Let's make this an lstlisting, not a figure...
\begin{lrbox}{}
\begin{lstlisting}[language=kotlin, style=nasm, xrightmargin=.6667\linewidth]
class Foo(var member: Int) 
{
  fun increment(N: Int): Int
  {
    member = member + N
    return member
  }
}

\end{lstlisting}
\end{lrbox}
\subcaptionbox{Kotlin Code\label{lst:kotlin}}{\usebox{\verbsavebox}}\hfill%
\begin{lrbox}{\verbsavebox}
\begin{lstlisting}[language=jimple, style=nasm, xrightmargin=.6667\linewidth]
public class Foo
{
  private int member;
  ...
  public int increment(int)
  {
    Foo r0;
    int i0, $i1, $i2, $i3;
    r0 := @this: Foo;
    i0 := @parameter0: int;
    $i1 = r0
      .<Foo: int member>;
    $i2 = $i1 + i0;
    r0.<Foo: int member>
      = $i2;
    $i3 = r0
      .<Foo: int member>;
    return $i3;
  }
}
\end{lstlisting}
\end{lrbox}
\subcaptionbox{Jimple Code (simplified)\label{lst:jimple}}{\usebox{\verbsavebox}}\hfill%
\begin{lrbox}{\verbsavebox}
\begin{lstlisting}[xrightmargin=.6667\linewidth]
trait Sys {
  type ID <: Ident[Tx]
  type Tx
}

trait Muta[S <: Sys] {
  // evidence required:
  val s: S
  def id: s.ID
  // well defined:
  def dispose(tx: s.Tx) =
    id.dispose(tx)
}
\end{lstlisting}
\end{lrbox}
\subcaptionbox{GOTO Code\label{lst:goto}}{\usebox{\verbsavebox}}
\caption{Kotlin into GOTO convertion\label{lst:example}}
\end{figure*}
